Why We Read Wikipedia

Wikipedia is one of the most popular sites on the Web, with millions of users relying on it to satisfy a broad range of information needs every day. Although it is crucial to understand what exactly these needs are in order to be able to meet them, little is currently known about why users visit Wikipedia. The goal of this paper is to fill this gap by combining a survey of Wikipedia readers with a log-based analysis of user activity. Based on an initial series of user surveys, we build a taxonomy of Wikipedia use cases along several dimensions, capturing users' motivations to visit Wikipedia, the depth of knowledge they are seeking, and their knowledge of the topic of interest prior to visiting Wikipedia. Then, we quantify the prevalence of these use cases via a large-scale user survey conducted on live Wikipedia with almost 30,000 responses. Our analyses highlight the variety of factors driving users to Wikipedia, such as current events, media coverage of a topic, personal curiosity, work or school assignments, or boredom. Finally, we match survey responses to the respondents' digital traces in Wikipedia's server logs, enabling the discovery of behavioral patterns associated with specific use cases. For instance, we observe long and fast-paced page sequences across topics for users who are bored or exploring randomly, whereas those using Wikipedia for work or school spend more time on individual articles focused on topics such as science. Our findings advance our understanding of reader motivations and behavior on Wikipedia and can have implications for developers aiming to improve Wikipedia's user experience, editors striving to cater to their readers' needs, third-party services (such as search engines) providing access to Wikipedia content, and researchers aiming to build tools such as recommendation engines.

==> results_material.tex <==
\newpage
\section{Full Results, not to be included}




\begin{table*}[b!]
	\small
	\centering
	\caption{\emph{Subgroup Discovery Results for motivations.} Each of the tables shows the subgroups that have significantly different share of users with a certain motivation. 
	For each result subgroup S, we display the size of the subgroup $P(S)$, i.e., the share of users that are covered by the subgroup description,  the coverage of this motivation by the subgroup ($P(S|T)$), the target share in the subgroup (\emph{P(T|S)}), i.e., the share of users within the subgroup that reported the respective motivation.
	For comparison, it also shows the respective share of users with this motivation in the entire user population (\emph{$P(T|S)$}), which is constant for all subgroups.}
	\subfloat[motivation = work/school]{\input{tables/sg_all_motivationworkschool_table}\label{table:sg3}} 
	\subfloat[motivation = media]{\input{tables/sg_all_motivationmedia_table.tex}\label{table:sg5}} \\
	\subfloat[motivation = personal decision]{\input{tables/sg_all_motivationpersonaldecision_table.tex}\label{table:sg4}} 
	\subfloat[motivation = intrinsic learning]{\input{tables/sg_all_motivationintrinsiclearning_table.tex}\label{table:sg6}}
\end{table*}	
	
\begin{table*}[b!]
	\small
	\centering
	\caption{\emph{Subgroup Discovery Results for motivations. continued.} Each of the tables shows the subgroups that have significantly different share of users with a certain motivation. 
	For each result subgroup S, we display the size of the subgroup $P(S)$, i.e., the share of users that are covered by the subgroup description,  the coverage of this motivation by the subgroup ($P(S|T)$), the target share in the subgroup (\emph{P(T|S)}), i.e., the share of users within the subgroup that reported the respective motivation.
	For comparison, it also shows the respective share of users with this motivation in the entire user population (\emph{$P(T|S)$}), which is constant for all subgroups.}	
	\subfloat[motivation = current event]{\input{tables/sg_all_motivationcurrentevent_table.tex}\label{table:sg7}}
	\subfloat[motivation = bored/random]{\input{tables/sg_all_motivationboredrandom_table.tex}\label{table:sg9}} \\
	\subfloat[motivation = conversation]{\input{tables/sg_all_motivationconversation_table.tex}\label{table:sg8}}
	\label{table:sgs_motivation}
\end{table*}

\begin{table*}[b!]
	\small
	\centering
	\caption{\emph{Subgroup Discovery Results for information need.}
	Each of the tables shows the 5 subgroups that have the most significantly increased share of users with a certain information need. 
	For each finding, we display the size of the subgroup, i.e., the share of users that are covered by the subgroup description, and the target share in the subgroup (\emph{Target(SG)}), i.e., the share of users within the subgroup that reported the respective information need.
	For comparison, it also shows the respective share of users with this motivation in the entire user population (\emph{Target(data)}), which is constant for all subgroups.} 
	\subfloat[information need = in-depth]{\input{tables/sg_all_informationdepth=indepth_table.tex}\label{table:sg11}} 
	\subfloat[information need = overview]{\input{tables/sg_all_informationdepth=overview_table.tex}\label{table:sg12}} \\
	\subfloat[information need = fact]{\input{tables/sg_all_informationdepth=fact_table}\label{table:sg13}} 
\end{table*}

\begin{table*}[b!]
	\small
	\centering
	\caption{\emph{Subgroup Discovery Results for prior knowledge.}
	Each of the tables shows the 5 subgroups that have the most significantly increased share of users with a prior knowledge. 
	For each finding, we display the size of the subgroup, i.e., the share of users that are covered by the subgroup description, and the target share in the subgroup (\emph{Target(SG)}), i.e., the share of users within the subgroup that reported the respective prior knowledge.
	For comparison, it also shows the respective share of users with this motivation in the entire user population (\emph{Target(data)}), which is constant for all subgroups.}
	\subfloat[prior knowledge = familiar]{\input{tables/sg_all_priorknowledge=familiar_table.tex}\label{table:sg21}} 
	\subfloat[prior knowledge = unfamiliar]{\input{tables/sg_all_priorknowledge=unfamiliar_table.tex}\label{table:sg22}} \\
\end{table*}

==> sg_all_informationdepth=fact_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                                Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                topic (tv, movies, novels) & 34.1\% &  36.8\% &  40.6\% &  1.08 &   ** \\
 \# referer ext. nonsearch (session): [0:1[ & 96.2\% &  97.4\% &  38.1\% &  1.01 &  *** \\
                       topic entropy>=2.69 & 20.0\% &  17.9\% &  33.7\% &  0.90 &    * \\
        topic (education, government, law) & 16.9\% &  14.6\% &  32.4\% &  0.86 &  *** \\
                            continent=Asia & 14.9\% &  11.9\% &  30.2\% &  0.80 &  *** \\
                           country code=IN & 13.5\% &  10.7\% &  29.8\% &  0.79 &  *** \\
                         referer: external &  3.2\% &   2.2\% &  25.8\% &  0.68 &   ** \\
     \# referer ext. nonsearch (session)>=1 &  3.8\% &   2.6\% &  25.2\% &  0.67 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_informationdepth=indepth_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                 Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
            country code=IN & 13.5\% &  20.9\% &  33.1\% &  1.55 &  *** \\
             continent=Asia & 14.9\% &  22.5\% &  32.4\% &  1.51 &  *** \\
 topic (tv, movies, novels) & 34.1\% &  29.9\% &  18.8\% &  0.88 &   ** \\
            country code=GB & 11.8\% &   9.2\% &  16.8\% &  0.79 &    * \\
           continent=Europe & 16.1\% &  12.5\% &  16.6\% &  0.77 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_informationdepth=overview_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                                Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                         referer: external &  3.2\% &   4.3\% &  52.4\% &  1.36 &  *** \\
     \# referer ext. nonsearch (session)>=1 &  3.8\% &   5.1\% &  51.4\% &  1.33 &  *** \\
        topic (education, government, law) & 16.9\% &  19.3\% &  43.9\% &  1.14 &  *** \\
                              host=desktop & 35.5\% &  40.1\% &  43.5\% &  1.13 &  *** \\
 \# referer ext. nonsearch (session): [0:1[ & 96.2\% &  94.9\% &  38.1\% &  0.99 &  *** \\
                           host=mobile web & 64.5\% &  59.9\% &  35.9\% &  0.93 &  *** \\
                            continent=Asia & 14.9\% &  12.4\% &  32.1\% &  0.83 &  *** \\
                           country code=IN & 13.5\% &  11.2\% &  32.0\% &  0.83 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationboredrandom_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                                Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                         referer: internal &  9.4\% &  14.0\% &  29.0\% &  1.49 &  *** \\
                 \# viewed pages in week>=8 & 11.8\% &  16.6\% &  27.5\% &  1.41 &  *** \\
                            topic (sports) &  5.9\% &   8.0\% &  26.1\% &  1.34 &   ** \\
             \# internal refers(session)>=1 & 17.1\% &  22.7\% &  25.9\% &  1.33 &  *** \\
             ses rel position: [0.33:0.75[ &  7.5\% &   9.8\% &  25.6\% &  1.31 &   ** \\
       avg. topic distance (session)>=1.08 &  7.5\% &   9.8\% &  25.2\% &  1.29 &    * \\
                      topic (21st century) & 25.1\% &  32.1\% &  25.0\% &  1.28 &  *** \\
              \# viewed pages in session>=3 & 22.2\% &  28.3\% &  24.8\% &  1.27 &  *** \\
 avg. time per page (session): [0.68:1.56[ &  7.7\% &   9.7\% &  24.7\% &  1.27 &    * \\
                      \# no referer(ses)>=2 &  9.7\% &  12.2\% &  24.5\% &  1.26 &    * \\
                topic (tv, movies, novels) & 34.1\% &  41.4\% &  23.7\% &  1.21 &  *** \\
                \# article pageviews>=63606 & 19.8\% &  23.5\% &  23.1\% &  1.19 &   ** \\
                   continent=North America & 63.4\% &  69.3\% &  21.3\% &  1.09 &  *** \\
                           country code=US & 57.1\% &  62.3\% &  21.3\% &  1.09 &  *** \\
         \# internal refers(session): [0:1[ & 82.9\% &  77.3\% &  18.2\% &  0.93 &  *** \\
          \# viewed pages in session: [1:2[ & 61.7\% &  57.0\% &  18.0\% &  0.92 &   ** \\
              session duration: [0.0:0.02[ & 62.0\% &  57.1\% &  18.0\% &  0.92 &  *** \\
         referer: external (search engine) & 62.6\% &  55.4\% &  17.3\% &  0.89 &  *** \\
                  article text length<6233 & 20.0\% &  16.7\% &  16.3\% &  0.84 &    * \\
                topic (biology, chemistry) &  8.6\% &   5.2\% &  11.8\% &  0.60 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationconversation_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                       Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
    \# viewed pages in week: [1:2[ & 48.3\% &  53.1\% &  24.4\% &  1.10 &  *** \\
 \# viewed pages in session: [1:2[ & 61.7\% &  66.7\% &  24.0\% &  1.08 &  *** \\
     session duration: [0.0:0.02[ & 62.0\% &  66.9\% &  23.9\% &  1.08 &  *** \\
                  host=mobile web & 64.5\% &  69.4\% &  23.9\% &  1.08 &  *** \\
                     host=desktop & 35.5\% &  30.6\% &  19.1\% &  0.86 &  *** \\
 \# external searches (session)>=2 & 20.5\% &  17.1\% &  18.6\% &  0.84 &   ** \\
     ses rel position: [0.0:0.33[ & 15.2\% &  12.5\% &  18.3\% &  0.82 &    * \\
     \# viewed pages in session>=3 & 22.2\% &  18.0\% &  17.9\% &  0.81 &  *** \\
        \# viewed pages in week>=8 & 11.8\% &   9.4\% &  17.7\% &  0.80 &    * \\
           session duration>=6.60 & 18.0\% &  13.7\% &  16.9\% &  0.76 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationcurrentevent_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                         Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                  topic (east asia) &  1.8\% &   3.6\% &  25.7\% &  2.03 &  *** \\
                     topic (sports) &  5.9\% &  11.7\% &  25.0\% &  1.97 &  *** \\
         \# article pageviews>=63606 & 19.8\% &  33.3\% &  21.3\% &  1.68 &  *** \\
               topic (21st century) & 25.1\% &  37.4\% &  18.9\% &  1.49 &  *** \\
 topic (education, government, law) & 16.9\% &  25.3\% &  18.9\% &  1.49 &  *** \\
                     continent=Asia & 14.9\% &  21.3\% &  18.2\% &  1.44 &  *** \\
                    country code=IN & 13.5\% &  19.3\% &  18.1\% &  1.43 &  *** \\
             article outdegree>=390 & 20.0\% &  26.3\% &  16.6\% &  1.31 &  *** \\
         article text length>=44860 & 20.0\% &  24.9\% &  15.8\% &  1.24 &   ** \\
         topic entropy: [2.42:2.69[ & 20.0\% &  24.1\% &  15.3\% &  1.21 &    * \\
               article outdegree<50 & 19.8\% &  15.7\% &  10.0\% &  0.79 &    * \\
                 topic entropy<1.87 & 20.0\% &  15.6\% &   9.9\% &  0.78 &   ** \\
           \# article pageviews<2519 & 19.8\% &  14.4\% &   9.2\% &  0.73 &  *** \\
                 topic (technology) & 13.2\% &   8.9\% &   8.5\% &  0.67 &  *** \\
            topic (literature, art) & 10.1\% &   5.9\% &   7.4\% &  0.58 &  *** \\
         topic (biology, chemistry) &  8.6\% &   4.6\% &   6.8\% &  0.53 &  *** \\
                topic (mathematics) &  7.9\% &   3.9\% &   6.2\% &  0.49 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationintrinsiclearning_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                 Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
    topic (literature, art) & 10.1\% &  13.1\% &  32.8\% &  1.30 &  *** \\
        topic (mathematics) &  7.9\% &   9.8\% &  31.2\% &  1.24 &    * \\
         topic (technology) & 13.2\% &  16.0\% &  30.5\% &  1.21 &   ** \\
             continent=Asia & 14.9\% &  17.8\% &  30.1\% &  1.20 &   ** \\
            country code=IN & 13.5\% &  16.1\% &  30.0\% &  1.19 &   ** \\
       topic (21st century) & 25.1\% &  21.9\% &  22.0\% &  0.87 &   ** \\
           continent=Europe & 16.1\% &  13.8\% &  21.5\% &  0.85 &    * \\
 \# article pageviews>=63606 & 19.8\% &  16.6\% &  21.1\% &  0.84 &   ** \\
            country code=GB & 11.8\% &   8.6\% &  18.4\% &  0.73 &  *** \\
 topic (tv, movies, novels) & 34.1\% &  24.1\% &  17.8\% &  0.71 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationmedia_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                    Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
    topic (tv, movies, novels) & 34.1\% &  46.9\% &  43.4\% &  1.37 &  *** \\
          topic (21st century) & 25.1\% &  31.6\% &  39.9\% &  1.26 &  *** \\
    \# article pageviews>=63606 & 19.8\% &  23.1\% &  36.9\% &  1.17 &  *** \\
         article pagerank<0.50 & 20.0\% &  22.9\% &  36.1\% &  1.14 &  *** \\
      \# no referer(ses): [1:2[ & 21.5\% &  24.1\% &  35.5\% &  1.12 &   ** \\
                 referer: none & 24.8\% &  27.3\% &  34.8\% &  1.10 &    * \\
               host=mobile web & 64.5\% &  68.7\% &  33.7\% &  1.07 &  *** \\
      \# no referer(ses): [0:1[ & 68.8\% &  65.7\% &  30.2\% &  0.95 &   ** \\
                  host=desktop & 35.5\% &  31.3\% &  27.8\% &  0.88 &  *** \\
        article outdegree>=390 & 20.0\% &  17.2\% &  27.1\% &  0.86 &  *** \\
               country code=IN & 13.5\% &  11.4\% &  26.8\% &  0.85 &    * \\
                continent=Asia & 14.9\% &  12.5\% &  26.7\% &  0.84 &   ** \\
      \# article pageviews<2519 & 19.8\% &  16.5\% &  26.4\% &  0.83 &  *** \\
         article indegree>=731 & 19.9\% &  16.5\% &  26.2\% &  0.83 &  *** \\
        article pagerank>=9.98 & 20.0\% &  14.9\% &  23.6\% &  0.75 &  *** \\
         topic (United States) &  4.9\% &   3.3\% &  21.5\% &  0.68 &  *** \\
           topic (mathematics) &  7.9\% &   5.2\% &  20.8\% &  0.66 &  *** \\
 topic (geographical entities) &  5.4\% &   3.5\% &  20.5\% &  0.65 &  *** \\
    topic (biology, chemistry) &  8.6\% &   5.4\% &  19.8\% &  0.63 &  *** \\
            topic (technology) & 13.2\% &   8.1\% &  19.4\% &  0.61 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationother_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
              Subgroup S &  P(S) &  P(S|T) &  P(T|S) &  P(T) & sig. \\
\midrule
 \# article pageviews<795 &  8.3\% &   12.7\% &   12.2\% &  7.9\% &    * \\
\bottomrule
\end{tabular}


==> sg_all_motivationpersonaldecision_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                    Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
 topic (geographical entities) &  5.4\% &   8.4\% &  14.8\% &  1.54 &   ** \\
               country code=IN & 13.5\% &  19.9\% &  14.3\% &  1.48 &  *** \\
                continent=Asia & 14.9\% &  21.8\% &  14.1\% &  1.46 &  *** \\
            topic (technology) & 13.2\% &  17.4\% &  12.7\% &  1.32 &    * \\
          article outdegree<50 & 19.8\% &  24.8\% &  12.1\% &  1.25 &    * \\
       continent=North America & 63.4\% &  57.5\% &   8.8\% &  0.91 &    * \\
                topic (sports) &  5.9\% &   2.4\% &   3.8\% &  0.40 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_motivationworkschool_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                                Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                       topic (mathematics) &  7.9\% &  17.1\% &  34.8\% &  2.17 &  *** \\
                      topic (war, history) &  4.4\% &   9.6\% &  34.7\% &  2.16 &  *** \\
                        topic (technology) & 13.2\% &  23.7\% &  28.8\% &  1.79 &  *** \\
                topic (biology, chemistry) &  8.6\% &  14.0\% &  26.2\% &  1.63 &  *** \\
                              host=desktop & 35.5\% &  57.8\% &  26.1\% &  1.63 &  *** \\
                    article pagerank>=9.98 & 20.0\% &  32.4\% &  26.1\% &  1.62 &  *** \\
        avg. time per page (session)>=9.40 &  7.7\% &  11.5\% &  24.0\% &  1.50 &  *** \\
         ses avg pagerank difference<-4.35 &  7.6\% &  11.2\% &  23.6\% &  1.47 &  *** \\
                   topic (literature, art) & 10.1\% &  14.7\% &  23.5\% &  1.46 &  *** \\
 avg. time per page (session): [3.60:9.40[ &  7.7\% &  11.0\% &  23.1\% &  1.44 &  *** \\
          \# external searches (session)>=2 & 20.5\% &  28.5\% &  22.4\% &  1.39 &  *** \\
                    session duration>=6.60 & 18.0\% &  24.2\% &  21.6\% &  1.34 &  *** \\
                        topic entropy<1.87 & 20.0\% &  25.7\% &  20.6\% &  1.28 &  *** \\
                     article indegree>=731 & 19.9\% &  25.3\% &  20.4\% &  1.27 &  *** \\
      \# article pageviews: [2519.0:8740.0[ & 19.8\% &  24.2\% &  19.6\% &  1.22 &  *** \\
         referer: external (search engine) & 62.6\% &  75.1\% &  19.3\% &  1.20 &  *** \\
        topic (education, government, law) & 16.9\% &  20.3\% &  19.2\% &  1.20 &    * \\
                    article outdegree>=390 & 20.0\% &  24.0\% &  19.2\% &  1.20 &   ** \\
     \# article pageviews: [8740.0:22514.0[ & 19.8\% &  23.4\% &  19.0\% &  1.18 &    * \\
             article pagerank: [3.22:9.98[ & 20.0\% &  23.5\% &  18.9\% &  1.18 &    * \\
                  \# no referer(ses): [0:1[ & 68.8\% &  79.0\% &  18.4\% &  1.15 &  *** \\
 \# referer ext. nonsearch (session): [0:1[ & 96.2\% &  98.0\% &  16.4\% &  1.02 &   ** \\
                   continent=North America & 63.4\% &  58.6\% &  14.9\% &  0.92 &   ** \\
                           country code=US & 57.1\% &  52.0\% &  14.6\% &  0.91 &   ** \\
            article indegree: [36.0:120.0[ & 19.9\% &  16.3\% &  13.1\% &  0.82 &    * \\
                topic entropy: [1.87:2.17[ & 20.0\% &  15.4\% &  12.4\% &  0.77 &  *** \\
                \# article pageviews>=63606 & 19.8\% &  14.1\% &  11.4\% &  0.71 &  *** \\
             article pagerank: [0.50:1.30[ & 20.0\% &  14.1\% &  11.3\% &  0.70 &  *** \\
                      \# no referer(ses)>=2 &  9.7\% &   6.5\% &  10.9\% &  0.68 &   ** \\
                  \# no referer(ses): [1:2[ & 21.5\% &  14.4\% &  10.8\% &  0.67 &  *** \\
                           host=mobile web & 64.5\% &  42.2\% &  10.5\% &  0.65 &  *** \\
                     article pagerank<0.50 & 20.0\% &  13.0\% &  10.4\% &  0.65 &  *** \\
                             referer: none & 24.8\% &  15.2\% &   9.9\% &  0.61 &  *** \\
      \# external searches (session): [0:1[ & 27.4\% &  16.1\% &   9.4\% &  0.59 &  *** \\
     \# referer ext. nonsearch (session)>=1 &  3.8\% &   2.0\% &   8.3\% &  0.52 &   ** \\
                topic (tv, movies, novels) & 34.1\% &  15.7\% &   7.4\% &  0.46 &  *** \\
                         referer: external &  3.2\% &   1.4\% &   7.1\% &  0.44 &   ** \\
                      topic (21st century) & 25.1\% &  10.5\% &   6.7\% &  0.42 &  *** \\
                             topic (music) &  9.3\% &   3.5\% &   6.0\% &  0.37 &  *** \\
                            topic (sports) &  5.9\% &   2.2\% &   5.8\% &  0.36 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_priorknowledge=familiar_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                                 Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
                             topic (sports) &  5.9\% &   7.2\% &  60.8\% &  1.21 &  *** \\
 avg. topic distance (session): [0.24:0.47[ &  7.6\% &   8.6\% &  56.8\% &  1.13 &    * \\
                     article outdegree>=390 & 20.0\% &  22.2\% &  55.6\% &  1.11 &  *** \\
                 \# article pageviews>=63606 & 19.8\% &  21.9\% &  55.5\% &  1.11 &  *** \\
                 article text length>=44860 & 20.0\% &  22.0\% &  55.1\% &  1.10 &  *** \\
                      article indegree>=731 & 19.9\% &  21.6\% &  54.4\% &  1.09 &   ** \\
                     article pagerank>=9.98 & 20.0\% &  21.6\% &  54.3\% &  1.08 &    * \\
                       topic (21st century) & 25.1\% &  27.0\% &  54.0\% &  1.08 &   ** \\
                 topic (tv, movies, novels) & 34.1\% &  36.7\% &  53.8\% &  1.07 &  *** \\
                    continent=North America & 63.4\% &  65.6\% &  51.9\% &  1.04 &   ** \\
                            country code=US & 57.1\% &  59.1\% &  51.9\% &  1.03 &    * \\
                        article indegree<36 & 19.7\% &  17.9\% &  45.4\% &  0.91 &   ** \\
                   article text length<6233 & 20.0\% &  18.0\% &  45.1\% &  0.90 &  *** \\
                       article outdegree<50 & 19.8\% &  17.5\% &  44.3\% &  0.88 &  *** \\
                        topic entropy>=2.69 & 20.0\% &  17.6\% &  44.2\% &  0.88 &  *** \\
\bottomrule
\end{tabular}


==> sg_all_priorknowledge=unfamiliar_table.tex <==
\begin{tabular}{lrrrrl}
\toprule
                 Subgroup S &  P(S) & P(S|T) & P(T|S) &  lift & sig. \\
\midrule
        topic entropy>=2.69 & 20.0\% &  22.5\% &  53.2\% &  1.12 &  *** \\
       article outdegree<50 & 19.8\% &  22.2\% &  53.1\% &  1.12 &  *** \\
        article indegree<36 & 19.7\% &  21.7\% &  52.1\% &  1.10 &   ** \\
   article text length<6233 & 20.0\% &  21.8\% &  51.5\% &  1.09 &    * \\
       topic (21st century) & 25.1\% &  23.3\% &  43.9\% &  0.93 &    * \\
 topic (tv, movies, novels) & 34.1\% &  31.6\% &  43.8\% &  0.93 &  *** \\
     article pagerank>=9.98 & 20.0\% &  18.3\% &  43.4\% &  0.92 &    * \\
      article indegree>=731 & 19.9\% &  18.1\% &  43.0\% &  0.91 &   ** \\
 article text length>=44860 & 20.0\% &  18.1\% &  42.7\% &  0.90 &   ** \\
 \# article pageviews>=63606 & 19.8\% &  17.8\% &  42.6\% &  0.90 &   ** \\
     article outdegree>=390 & 20.0\% &  17.9\% &  42.2\% &  0.89 &  *** \\
             topic (sports) &  5.9\% &   4.6\% &  36.8\% &  0.78 &  *** \\
\bottomrule
\end{tabular}


==> survey_crosstable_depth_prior.tex <==
\begin{tabular}{lrrr}
\toprule
prior knowledge &  familiar &  no response &  unfamiliar \\
information depth &           &              &             \\
\midrule
fact              &    0.5729 &       0.0098 &      0.4173 \\
in-depth          &    0.5765 &       0.0120 &      0.4115 \\
no response       &    0.1544 &       0.7046 &      0.1410 \\
overview          &    0.4183 &       0.0070 &      0.5747 \\
\bottomrule
\end{tabular}


==> survey_crosstable_motivation_depth.tex <==
\begin{tabularx}{0.45\textwidth}{l|XXX|l} 
\toprule 
information depth & fact & in-depth & overview & sig. \\ 
motivation &  &  &  &  \\ 
\midrule 
bored/random & 0.3077 & 0.2146 & 0.4653 & *** \\ 
conversation & 0.4153 & 0.1966 & 0.3776 & *** \\ 
current event & 0.3711 & 0.2672 & 0.349 & *** \\ 
intrinsic learning & 0.2918 & 0.3396 & 0.3565 & *** \\ 
media & 0.3682 & 0.1893 & 0.4358 & *** \\ 
other & 0.4001 & 0.2022 & 0.3279 & *** \\ 
personal decision & 0.341 & 0.2783 & 0.3646 & *** \\ 
work/school & 0.3854 & 0.2459 & 0.3543 & *** \\ 
\hline 
response perc. & 0.3664 & 0.2205 & 0.389 & \\ 
\bottomrule 
\end{tabularx} 


==> survey_crosstable_prior_depth.tex <==
\begin{tabularx}{0.45\textwidth}{l|XXX|l} 
\toprule 
information depth & fact & in-depth & overview & sig. \\ 
prior knowledge &  &  &  &  \\ 
\midrule 
familiar & 0.4174 & 0.2522 & 0.323 & *** \\ 
unfamiliar & 0.3249 & 0.1929 & 0.4757 & *** \\ 
\hline 
response perc. & 0.3664 & 0.2205 & 0.389 & \\ 
\bottomrule 
\end{tabularx} 

